Learning to Bound the Multi-class Bayes Error

In the context of supervised learning, meta learning uses features, metadata and other information to learn about the difficulty, behavior, or composition of the problem. Using this knowledge can be useful to contextualize classifier results or allow for targeted decisions about future data sampling. In this paper, we are specifically interested in learning the Bayes error rate (BER) based on a labeled data sample. Providing a tight bound on the BER that is also feasible to estimate has been a challenge. Previous work[1] has shown that a pairwise bound based on the sum of Henze-Penrose (HP) divergence over label pairs can be directly estimated using a sum of Friedman-Rafsky (FR) multivariate run test statistics. However, in situations in which the dataset and number of classes are large, this bound is computationally infeasible to calculate and may not be tight. Other multi-class bounds also suffer from computationally complex estimation procedures. In this paper, we present a generalized HP divergence measure that allows us to estimate the Bayes error rate with log-linear computation. We prove that the proposed bound is tighter than both the pairwise method and a bound proposed by Lin [2]. We also empirically show that these bounds are close to the BER. We illustrate the proposed method on the MNIST dataset, and show its utility for the evaluation of feature reduction strategies. We further demonstrate an approach for evaluation of deep learning architectures using the proposed bounds.

==> BERbound.tex <==
\section{BOUNDS ON THE BAYES ERROR RATE}\label{Sec.BERbounds}
Before introducing the new bound on multi-class BER, we first review the pairwise bounds on the multi-class Bayes error rate given by Berisha et al. \cite{BerishaICassp2016} and by Lin \cite{Lin1991}. %Using methods in \cite{Berishaetal2016}, the authors in \cite{BerishaICassp2016} generalized binary classification bound based on the HP-divergence to multi-class problems.
\subsection{Pairwise HP Bound}
For the case of $m$ classes the authors in \cite{BerishaICassp2016} have shown that the multi-class BER $\epsilon^m$ in (\ref{BER.m-classes}) can be bounded by
\begin{equation}\label{multiclass.HP-bound}\begin{array}{l}
\diy\frac{2}{m}\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m (p_i+p_j)\epsilon_{ij}\leq \epsilon^m\leq \diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m (p_i+p_j)\epsilon_{ij},
\end{array}\end{equation}
where $\epsilon_{ij}$ represents the pairwise Bayes risk of the two class sub-problem of classifying between classes $i$ and $j$:
\begin{equation}
\epsilon_{ij}=\diy\int \min \big\{\widetilde{p}_{ij}f_{i}(\bx),\widetilde{p}_{ji}f_{j}(\bx)\big\}\;\rd\bx.
\end{equation}
%where 
%\begin{equation}\label{def.tildP}
%\widetilde{p}_{ij}=p_i\big/(p_i+p_j)\;\;\;\hbox{and}\;\;\; \widetilde{p}_{ji}=p_j\big/(p_i+p_j).\end{equation}
%Note that $\widetilde{p}_{ij}\neq \widetilde{p}_{ji}$ and $\widetilde{p}_{ij}+ \widetilde{p}_{ji}=1$. 
In \cite{Berishaetal2016}, it has been shown that
\begin{equation}\label{Berisha.bound}
\diy\frac{1}{2}-\frac{1}{2} \sqrt{u_{\widetilde{p}_{ij}}(f_{i},f_{j}})\leq \epsilon_{ij}\leq \diy\frac{1}{2}-\frac{1}{2}u_{\widetilde{p}_{ij}}(f_{i},f_{j}), 
\end{equation}
%where 
\begin{equation}\label{expression:U}
\hbox{where}\;\;u_{\widetilde{p}_{ij}}(f_{i},f_{j})=4\widetilde{p}_{ij}\widetilde{p}_{ji}\; D(f_{i},f_{j})+(\widetilde{p}_{ij}-\widetilde{p}_{ji})^2,
\end{equation}
and $D(f_i,f_j)$ is defined in (\ref{EQ:DP}). Using both (\ref{multiclass.HP-bound}) and (\ref{Berisha.bound}), we obtain bounds for the multi-class Bayes error rate. While these bounds have been successfully applied \cite{FR}, \cite{Berishaetal2016}, it has the disadvantage of high computational complexity due to the presence of ${m \choose 2}$ summands in (\ref{multiclass.HP-bound}).
%In order to compute the pairwise HP-bound, $m(m-1)/2$ MSTs must be computed.
\def\bbE{\mathbb{E}}
\subsection{JS Bound}
The generalized Jensen-Shannon divergence is defined as 
$$JS(f_1,f_2,\dots,f_m)=\bar{H}\left(\diy\sum\limits_{k=1}^m p_kf_k\right)-\diy\sum\limits_{k=1}^m p_i\bar{H}(f_i), $$
where $\bar{H}$ is the Shannon entropy function.
%$$\bar{H}(f)=-\diy\int f(\bx)\log f(\bx)\;\rd\bx.$$ 
In \cite{Lin1991} this divergence measure was used to obtain a bound on the multi-class BER. The Bayes error rate $\epsilon^m$ is upper bounded by
\begin{equation}\label{Upper-Lin}
\epsilon^m\leq\diy\frac{1}{2}\big(H(p)-JS(f_1,f_2,\dots,f_m)\big):=\epsilon^m_{\rm JS} \;\;\hbox{(say)},
\end{equation}
and is lower bounded by 
%$\epsilon^m\geq \diy\big(\epsilon^m_{\rm JS}\big)^2/(m-1)$.
\begin{equation}\label{JS:lowerbound}
\epsilon^m\geq \diy\frac{1}{4(m-1)}\big(H(p)-JS(f_1,f_2,\dots,f_m)\big)^2.
\end{equation}
Here $H(p)$
%$H(p)=-\diy\sum\limits_{k=1}^m p_k\log p_k$ 
is Shannon entropy and $JS$ is generalized Jensen-Shannon divergence. The bounds in (\ref{Upper-Lin}) and (\ref{JS:lowerbound}) can be approximated by plug-in estimation or by direct methods, such as the NNR method \cite{NMYH} or other graph methods \cite{Heroetal2002}. We will show that the JS bound suffers from lack of tightness.

%is that to the best of our knowledge except applying NNR estimator introduced in \cite{MortezaISIT2017}, the plug-in approaches are only methods that can be used to approximate them. This is very expensive and for large number of classes less accurate. 


%------------------------------------------------
\subsection{Proposed Multi-class Bayes Error Probability Bound}
%In this work we introduce a new upper bound, which we call the generalized Henze-Penrose (GHP) bound which is provably tighter than the pairwise HP bound and the JS bound. 
%Denote
%$$\gamma_l=\max\{p_1f_1,p_2f_2,\dots,p_lf_l\}.$$
%we make the following assumption regarding the joint distributions $p_kf_k$, for $k=1,2\dots,m$.
 
%{\bf Assumption 1:} For given priors $p_1,p_2,\dots,p_m$ and conditional probability densities we have
%\begin{equation}\label{main.assumtion}\begin{array}{l}
%\diy\int\max\Big\{\gamma_{m-2}(\bx),p_{m-1}f_{m-1}(\bx),p_mf_m(\bx)\Big\}\rd\bx\\
%\qquad\geq \diy\int \max\Big\{\gamma_{m-2},p_{m-1}f_{m-1}(\bx)+p_mf_m(\bx)\Big\}\;\rd\bx\\
%\qquad\qquad-\diy\int\min\Big\{p_{m-1}f_{m-1}(\bx),p_{m}f_m(\bx)\Big\}\rd\bx.
%\end{array}\end{equation}
To simplify notation, denote
$$
\delta_{ij}:=\diy\int \diy\frac{p_i p_j f_i(\bx)f_j(\bx)}{p_if_i(\bx)+p_jf_j(\bx)}\rd\bx,\;\;\;{\it\delta^m_{ij}:= \diy\int \diy\frac{p_i p_j f_i(\bx)f_j(\bx)}{f^{(m)}(\bx)}\rd\bx}, 
$$

and note that 
%$2 \delta_{ij} = \frac{1}{2}-\frac{1}{2}u_{p_{ij}}(f_{i},f_{j})$
$ \delta_{ij} = \frac{(p_i+p_j)}{4}\big(1-u_{\widetilde{p}_{ij}}(f_{i},f_{j})\big)$, where $u_{\widetilde{p}_{ij}}$ is defined in (\ref{expression:U}) and $\delta_{ij} \geq \delta_{ij}^{m}$.
%Furthermore, $\delta_{ij}=p_ip_j {\rm HP}_{ij}$ 

%And $\Delta(h_1,h_2):=\diy\int h_1(\bx)\log \diy\frac{h_1(\bx)}{h_2(\bx)}\;\rd\bx$, where $h_1$ and $h_2$ are non-negative functions and $h_2\neq 0$. Note that $\Delta$ becomes KL-divergence when $h_1$ and $h_2$ are probability density function. 
\begin{theorem}\label{thm.2} 
{\it For given priors $p_1,p_2,\dots,p_m$ and conditional distributions $f_1,f_2,\dots,f_m$, 
%\begin{equation}\label{assum.1}\begin{array}{cl}
%2 \delta_{ij}
%\leq 2\delta^m_{ij}
%\end{array}\end{equation}
the multi-class BER $\ep^m$ satisfies 
\begin{equation}\label{proposed.upbound}
\ep^m\leq 2\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta^m_{ij}.
\end{equation}
And is lower bounded by $\delta^m_{ij}$ as
\begin{equation}\label{lowerbound.2}
\ep^m\geq \diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right].
\end{equation}
}
\end{theorem}
{\bf Proof Sketch:}
To derive (\ref{proposed.upbound}) and (\ref{lowerbound.2}) we first show that for a probability distribution on $m$ classes, $a_1,a_2,\dots,a_m$ such that $\diy\sum\limits_{i=1}^m a_i=1$, we have
$1-\max\limits_i a_i\leq 2\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^{m} a_i a_j,$
\begin{equation}
\diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} a_i a_j\right)^{1/2}\right] \le 1 - \max_i a_i,
\end{equation}
respectively. Then by setting $a_i=p(i|\bx):=P(y=i|\bx)$ and the fact that the BER for $m$ classes is given by 
$$\epsilon^m=\bbE_\BX\Big[1-\max\limits_{i=1,\dots,m} p(i|\bx)\Big],$$
we complete the proof. 
In the following theorem we show that the proposed upper and lower bounds are tighter than the JS upper (\ref{Upper-Lin}) and lower (\ref{JS:lowerbound}) bounds.
\begin{theorem}\label{GHPandJS.upbound}
{\it For given priors $p_1,p_2,\dots,p_m$ and conditional distributions $f_1,f_2,\dots,f_m$, for $m\geq 3$
\begin{equation}\label{Ineq:tighterJS}
\ep^m\leq 2\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta^m_{ij}\leq
\epsilon^m_{\rm JS},
%\diy\frac{1}{2}\big(H(p)-JS(f_1,f_2,\dots,f_m)\big), \;\hbox{and}
\end{equation}
\begin{equation}\label{lowerbound.1.tight}\begin{array}{l}
\ep^m\geq \diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right]\geq \diy \frac{(\epsilon^m_{\rm JS})^2}{(m-1)}.
%\\
%\qquad \geq \diy\frac{1}{4(m-1)}\big(H(p)-JS(f_1,f_2,\dots,f_m)\big)^2.
\end{array}\end{equation}
}
\end{theorem}
{\bf Proof Sketch:} To prove tightness (\ref{Ineq:tighterJS}) and (\ref{lowerbound.1.tight}), we establish two inequalities:
\begin{equation*}\begin{array}{cl}
2\diy\sum_{i=1}^{m-1}\sum_{j=i+1}^m a_i a_j\leq -\diy\frac{1}{2} \sum_{i=1}^m a_i\log a_i,\\
 \diy\bbE_{\BX}\left[\sum_{i=1}^{m-1} \sum_{j=i+1}^{m} a_i a_j\right]\geq \diy\frac{1}{4(m-1)} \left(\bbE_\BX\left[\sum\limits_{i=1}^m a_i\log a_i\right]\right)^2,
\end{array}\end{equation*}
respectively. These inequalities are key points to derive our claims along with rewriting (\ref{lowerbound.1.tight}) as 
\begin{equation*}
    \diy\frac{m-1}{m}\left[ 1 -\sqrt{\bbE_\BX[A(\BX)]}\right]\geq \diy\frac{1}{4(m-1)}\left(\bbE_\BX\left[\sum\limits_{i=1}^m a_i\log a_i\right]\right)^2,
\end{equation*}
where $A(\bx)=1 - 2\frac{m}{m-1}\left[\sum_{i=1}^{m-1} \sum_{j=i+1}^{m} a_i a_j\right]. $
Now, analogous to Theorem \ref{thm.2}, by letting $a_i=p(i|\bx)$ we complete the proof.

%In the following, we derive a lower bound in terms of $\delta^m_{ij}$:
%\begin{theorem}\label{thm2:lowerbound2}
%For given priors $p_1,p_2,\dots,p_m$ and conditional distributions $f_1,f_2,\dots,f_m$, the multi-class classification BER $\ep^m$ is lower bounded by $\delta^m_{ij}$ as
%\begin{equation}\label{lowerbound.2}
%\ep^m\geq \diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right].
%\end{equation}
%\end{theorem}
%The proofs are given in Section \ref{sec.proofs}.
%----------------------------------------------------
%\begin{theorem}\label{thm.lower.tight.1}
%For given priors $p_1,p_2,\dots,p_m$ and conditional distributions $f_1,f_2,\dots,f_m$, the multi-class classification BER $\ep^m$ is lower bounded by $\delta^m_{ij}$ as
%\begin{equation}\label{lowerbound.1.tight}\begin{array}{l}
%\ep^m\geq \diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right]\\
%\\
%\qquad \geq \diy\frac{1}{4(m-1)}\big(H(p)-JS(f_1,f_2,\dots,f_m)\big)^2.
%\end{array}\end{equation}
%\end{theorem}
%----------------------------------------------------
Theorem~\ref{thm.lower.tight.2} shows that proposed upper and lower bounds are tighter than bounds in (\ref{multiclass.HP-bound}), i.e., the pairwise (PW) bounds. 
\begin{theorem}\label{thm.lower.tight.2}
{\it For given priors $p_1,p_2,\dots,p_m$ and conditional distributions $f_1,f_2,\dots,f_m$, the multi-class classification BER $\ep^m$ is upper bounded 
\begin{equation}\label{upper.toghterPW}
\ep^m\leq 2\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta^m_{ij}\leq 2\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta_{ij}. 
\end{equation}
and is lower bounded by $\delta^m_{ij}$ as
\begin{equation}\label{lowerbound.2.tight}\begin{array}{l}
\ep^m\geq \diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right]\\
\\
\qquad \geq \diy\frac{2}{m}\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m (p_i+p_j)\left[\diy\frac{1}{2}-\frac{1}{2} \sqrt{u_{\widetilde{p}_{ij}}(f_{i},f_{j}})\right].
\end{array}\end{equation}
where $u_{\widetilde{p}_{ij}}$ is given in (\ref{expression:U}). 
}
\end{theorem}
{\bf Proof Sketch:}
Similar to the proofs of Theorems \ref{thm.2} and \ref{GHPandJS.upbound}, the upper bound is easy to derive. The tightness claim for the lower bound requires to show that:
\begin{equation*}\begin{array}{l}
    \diy\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \diy \left((p_i+p_j)^2-\diy 4(p_i+p_j)\bbE_\BX\left[\frac{a_ia_j}{a_i+a_j}\right]\right)^{1/2}\\
    \qquad \geq \diy(m-1) \left(1 - 2\frac{m}{m-1} \bbE_\BX\left[\sum_{i=1}^{m-1} \sum_{j=i+1}^{m} a_i a_j\right]\right)^{1/2}. 
\end{array}\end{equation*}
by setting $a_i=p(i|\bx)$, this involves lower bound on the summed  posterior probabilities,
$$\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m p(i|\bx)p(j|\bx),$$
and establishes our claim in (\ref{lowerbound.2.tight}) and provides tighter upper and lower bound that those given in \cite{Lin1991} and \cite{BerishaICassp2016}.
The full proofs of Theorems \ref{thm.2}, \ref{GHPandJS.upbound}, and
\ref{thm.lower.tight.2} are given in the long version of the paper on arXiv
\cite{arXiv-Paper}.

In addition to the above Theorem, we are able to more precisely characterize the
relationship between the pairwise and GHP upper bounds:

\begin{proposition}
  \label{prop:1}
  The equality on the right hand side of (\ref{upper.toghterPW}) holds
%\begin{equation*}
 %2\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta^m_{ij}\leq 2\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta_{ij},
%\end{equation*}
%with equality holding 
iff a) $m=2$, or b) $\forall i \neq j, (\bS^{(i)} \cup
\bS^{(j)}) \cap \cup_{k \neq i, j} \bS^{(k)}=\emptyset$.
\end{proposition}

%The proof is given in the arXiv version~\cite{arXiv-Paper}.
%To derive the inequalities (\ref{proposed.upbound})-(\ref{lowerbound.2.tight}) a set of general inequalities for posterior probabilities $a_i:=p(i|\bx)$ are established. 

%The proof of the tightness results (\ref{Ineq:tighterJS})-(\ref{lowerbound.2.tight}) for JS and pairwise upper and lower bounds requires a different approach that involves deriving upper and lower bounds on the summed posterior probabilities,
%$$\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m p(i|\bx)p(j|\bx).$$
%This approach provides tighter upper and lower bound that those given in \cite{Lin1991} and \cite{BerishaICassp2016}. 
\begin{proposition}
  \label{prop:2}
   The equality on the right hand side of (\ref{lowerbound.2.tight}) holds
%\begin{equation}\label{lowerbound.2.tight-equality}
%\begin{array}{l}
%\diy\frac{m-1}{m}\left[ 1 - \left(1 - 2\frac{m}{m-1} \sum_{i=1}^{m-1} \sum_{j=i+1}^{m} \delta^m_{ij}\right)^{1/2}\right]\\
%\\
%\qquad \geq \diy\frac{2}{m}\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m (p_i+p_j)\left[\diy\frac{1}{2}-\frac{1}{2} \sqrt{u_{\widetilde{p}_{ij}}(f_{i},f_{j}})\right].
%\end{array}\end{equation}
%with equality holding 
iff $m=2$.
\end{proposition}

The proofs of Propositions \ref{prop:1} and \ref{prop:2} are given in the arXiv version~\cite{arXiv-Paper}.
%--------------------------------------------------------------
\section{Learning the bounds from data}\label{sec.estimate.delta}

%\subsubsection{The General Friedman-Rafsky (GFR) Statistics}
Here we review the pairwise Friedman-Rafsky (FR) statistic and introduce a generalized FR statistic. Given a labeled sample $\BX=\{(\mathbf{x}_i, y_i)\}_{i=1}^n$ define the subset of samples having label $k$ as: $\mathbf{X}^{(k)}=\{(\mathbf{x}_i, y_i)\}_{i=1,y_i=k}^n$, $k=1, \ldots, m$.  The cardinality of the subset $\mathbf{X}^{(k)}$ is $n_k=\sum_{i=1}^n I(y_i=k)$ where $I(B)$ denotes the indicator function of event $B$.  
%The sample realization from the $i$th class is denoted $\bx^{(i)}=\{\bx^{(i)}_1,\bx^{(i)}_2,\dots \bx^{(i)}_{n_i}\}$. 
We denote the pairwise FR statistic by $\mathfrak{R}_{n_i,n_j}$ and the generalized FR statistic by $\mathfrak{R}^{(ij)}_{n_1,n_j}$ that are computed as follows
\begin{itemize}
\item[1.] $\mathfrak{R}_{n_i n_j}:=\mathfrak{R}_{n_i n_j}(\BX)$ is the number of dichotomous edges in a Euclidean minimal spanning tree (MST) spanning the samples in the pairwise union of samples with labels $i$ and $j$ , $\BX^{(i)}\cup \BX^{(j)}\in \bbS^{(i)}\cup\bbS^{(j)}$, where $\BX^{(k)}=\{(\bx_i,y_i)\}_{i=1,Y_i=k}^n$. A dichotomous edge is an edge that connects a sample from class $i$ to a sample from class $j$. The pairwise FR statistic $\mathfrak{R}_{n_i n_j}$ for three classes is illustrated in Fig~\ref{fig:pairwiseghp_example}.  \\
\item[2.] $\mathfrak{R}^{(ij)}_{n_i,n_j}:=\mathfrak{R}^{(ij)}_{n_i,n_j}(\BX)$ is the number of dichotomous edges connecting a sample from class $i$ to a sample from class $j$ in the global MST constructed on all samples with all classes $1,2\ldots,m$ i.e. $\bigcup\limits_{k=1}^m \{(\bx_i,y_i)\}_{i=1,y_i=k}^n$ or  $\BX^{(1)}\cup\BX^{(2)}\cup\dots\cup\BX^{(m)}\in \bbS^{(1)}\cup \bbS^{(2)}\cup\dots \bbS^{(m)}$ where $\BX^{(k)}=\{(\bx_i,y_i)\}_{i=1,y_i=k}^n$, $k=1,\ldots,m$. Fig~\ref{fig:ghp_example} represents the generalized FR statistic for three classes. 
\end{itemize}
Using the theory in \cite{HP} and \cite{Berishaetal2016}, the estimator $\mathfrak{R}_{n_i,n_j}$ is a statistically consistent estimator of  the pairwise HP-bound for classifying class $i$ vs. class $j$. This yields an estimate of the bounds (11) on multi-class BER, requiring the construction of $m \choose 2$ MSTs spanning all distinct pairs of label classes. The next theorem implies that $\mathfrak{R}^{(ij)}_{n_i,n_j}$ can be used to estimate the tighter bound on multi-class BER given in Theorem \ref{thm.2} using only a single global MST. 
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/pairwise_example.pdf}
%\vspace{-0.8cm}
\caption{Estimating $\mathfrak{R}_{n_i,n_j}$ for three classes. A set of $m(m-1)/2$ Euclidean MSTs are computed for each unordered pair of classes $\{(i,j)\}_{i>j}$, and then the dichotomous edges (in red) are counted to find $\mathfrak{R}_{n_i,n_j}$.}
\label{fig:pairwiseghp_example}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=3.2in] {figs/general_example.pdf}
\caption{Estimating $\mathfrak{R}^{(ij)}_{n_i,n_j}$ for three classes. A single MST is constructed over all classes $i=1,2,3$ of points. For each $(i, j)$, count the edges connecting points from classes $i$ and $j$. These edges are shown in 3 different colors each corresponding to the three types of pairs $(i,j)=(1,2), (2,3), (1,3)$.}
\label{fig:ghp_example}
\end{figure}

\begin{theorem}\label{thm:5}
{\it Let $\mathbf X= \{(\bx_i, y_i)\}_{i=1}^n$ be an i.i.d. $m$-class labeled sample and $n_k=\sum_{i=1}^n I(y_i=k)$, be the cardinality of samples with label $k$. For distinct classes $i,j$ let $i,j=1,\dots, m$, $n_i,n_j\rightarrow \infty$, $n\rightarrow \infty$ such that $n_i/n\rightarrow p_i$ and $n_j/n\rightarrow p_j$. Then
\begin{equation} \label{eq:V} \diy\frac{\mathfrak{R}^{(ij)}_{n_i,n_j}(\BX)}{2n}\diy\longrightarrow \delta^m_{ij}\;\; \;\; \hbox{(a.s.)}\end{equation}
}
\end{theorem}
{\bf Proof Sketch:} The proof for Theorem~\ref{thm:5} uses arguments similar to  those used in~\cite{HP} to establish the convergence of the Friedman Rafsky two sample statistic, but generalized to more than two labeled populations. The idea is to incorporate Poission variables $N_{n_k}$ with mean  $n_k=\diy\sum_{i=1}^n I(y_i=k)$, for $k=1,\dots,m$ and independent of one another and of $\BX^{(k)}=\{(\bx_i,y_i)\}_{i=1,y_i=k}^n$. Next by Poissonization of data as $\overline{\BX}^{(k)}=\{(\bx_i,y_i)\}_{i=1,y_i=k}^{N_{n_k}}$ with FR statistic $\overline{\mathfrak{R}}^{(ij)}_{n_i,n_j}$, it is sufficient to show that $\diy \mathbb{E}\left[\overline{\mathfrak{R}}^{(ij)}_{n_i,n_j}\right]/(2n)\rightarrow \delta_{ij}^m$. To do this, we define a nonhomogeneous Poisson process and assign a mark from the set $\{1,2,\ldots,m\}$ to each point in this set. Next we construct global MST and count dichotomous edges with two different types of marks denoted by $\widetilde{\mathfrak{R}}^{(ij)}_{n_i,n_j}$. According to marking theorem marked points are independent Poisson process with the same distribution as the original Poisson points. Finally, using arguments similar to those in \cite{HP}, we establish that 
\begin{equation*} 
\diy \frac{\mathbb{E}\left[\widetilde{\mathfrak{R}}^{(ij)}_{n_i,n_j}\right]}{n}\rightarrow 2\diy\int \diy\frac{p_{i} p_{j} f_i(\bx) f_j(\bx)}{\diy\sum\limits_{k=1}^m p_k f_k(\bx)}\rd\bx. 
\end{equation*}
Furthermore, using arguments similar to those in \cite{YOH}, it is also possible to establish convergence of the cross-match statistic by running the optimal weighted matching graph over pairs of label classes. 
Details on the proof are given in the longer version of the paper posted on arXiv~\cite{arXiv-Paper}. 




==> Domain-Adaption.tex <==
\section{Domain adaption in multi-classification problem}\label{sec:dom_apt}
In this section, we formalize the problem of domain adaptation for multi-class classification as follows. 
Let us define data from two domains, the source (training) and the target (testing) domain and the corresponding label functions for each domain $y_S(\bx),\;y_T(\bx)\in\{1,\dots,m\}$ that yields the true class label of a given data point $\bx$. Then we show that the predicted classification accuracy on the unlabeled testing data is bounded by the predicted classification accuracy on training data. We denote by $(D_S,y_S)$ the source domain and $(D_T,y_T)$ the target domain.
The conditional distributions $f_{S,i}(\bx)$ and $f_{T,i}(\bx)$ are defined by $f_S(\bx|y_S(\bx)=i)$ and $f_T(\bx|y_T(\bx)=i)$, respectively for $i=1,\dots,m$ where the training and test data are drawn from distribution $f_S(\bx)$ and $f_T(\bx)$. Define 
$$f_S(\bx)=\diy\sum_{i=1}^m P(y_S(\bx)=i)f_{S,i}(\bx),$$
and similarly 
$$f_T(\bx)=\diy\sum_{i=1}^m P(y_T(\bx)=i)f_{T,i}(\bx).$$ 
A hypothesis is a function $h$ that takes values $\{1,\dots,m\}$ over the feature space. The probability according to the distribution $D_S$ that a hypothesis disagrees with the labeling function $y_S$ is defined as
\begin{equation}
    \epsilon_S(h,y_S)=\mathbb{E}_{f_S}\big[|h(\bx)-y_S(\bx)|\big]]. 
\end{equation}
Similarly  the probability according to the distribution $D_T$ that a hypothesis disagrees with the labeling function $y_T$ is given by
\begin{equation}
    \epsilon_T(h,y_T)=\mathbb{E}_{f_T}\big[|h(\bx)-y_T(\bx)|\big]]. 
\end{equation}
In \cite{Berishaetal2016}, it has been established that
\begin{equation}
    \epsilon_T(h,y_T)\leq \epsilon_S(h,y_S)+\mathbb{E}_{f_S}\big[|y_S-y_T|\big]+2\sqrt{u_{\frac{1}{2}}(f_S,f_T)},
\end{equation}
where 
$$u_{\frac{1}{2}}(f_S,f_T)=1-2\diy\int \frac{f_S(\bx)f_T(\bx)}{f_S(\bx)+f_T(\bx)}\;\rd\bx.$$
In the covariate shift scenario, we assume that there exists no difference between labeling functions (i.e. $y_S(\bx)=y_T(\bx)$. Further, if we assume that the decision rule $h$ attains the Bayes error rate on source domain $D_S$, we can write 
\begin{equation}\label{UB.Domain}
   \epsilon_T(h,y_T)\leq 2\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m \delta^m_{ij}(D_S)+2\sqrt{u_{\frac{1}{2}}(f_S,f_T)},
\end{equation}
where 
$$\delta^m_{ij}(D_S)= \diy\int \diy\frac{p_{S,i} p_{S,j} f_{S,i}(\bx)f_{S,j}(\bx)}{f_S(\bx)}\rd\bx,$$
and $p_{S,i}=P(y_S(\bx)=i)$. 
Denote $n_{S}$ and $n_{T}$ by the cardinality of $D_S$ and $D_T$. Let $n_{S,i}$ be sample size of source data with label $i$ and $\BX_{S}^{(i)}$ be the source data in domain $D_S$ ($\BX_S^{(i)}\in D_S$) with label $i$. By Theorem \ref{thm:5}, so we have 
\begin{equation} \diy\frac{\mathfrak{R}^{(ij)}_{n_{S,i},n_{S,j}}(\BX^{(i)}_S,\BX^{(j)}_S)}{2n_S}\diy\longrightarrow \delta^m_{ij}(D_S)\;\; \;\; \hbox{(a.s.)}\end{equation}
Applying Theorem 1 in \cite{Berishaetal2016}, we can estimate the upper bound in \ref{UB.Domain} using global and pairwise FR test statistic by
\begin{equation}
  \sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m   \diy\frac{\mathfrak{R}^{(ij)}_{n_{S,i},n_{S,j}}(\BX^{(i)}_S,\BX^{(j)}_S)}{n_S}+2\sqrt{1-2\diy\frac{\mathfrak{R}_{n_S,n_T}(D_S,D_T)}{n_S+n_T}},
\end{equation}
where $\mathfrak{R}_{n_S,n_T}(D_S,D_T)$ is the standard FR test statistic between source (training) and target (test) data following constructing MST over $D_S\cup D_T$. 

==> Extratheorems.tex <==
\subsection{Theorem \ref{thm1:lowerbound}}
Going back to generalized Jensen-Shannon divergence's definition, we can write
\begin{equation}\begin{array}{l}
JS(f_1,f_2,\dots,f_m)=\diy\sum\limits_{i=1}^m \int p_if_i(\bx)\log f_i(\bx)\;\rd\bx \\
\qquad-\int {\it f^m}(\bx)\log {\it f^m}(\bx)\;\rd\bx
={\it \diy\sum\limits_{i=1}^m p_i\int f_i(\bx)\log\diy\frac{f_i(\bx)}{f^m(\bx)}}\\
\qquad\qquad=\diy\sum\limits_{i=1}^m p_i \Delta\big(f_i,f^m\big), 
\end{array}\end{equation}
where for non-negative functions $h_1$, $h_2$ ($h_2\neq 0$),
$$\Delta(h_1,h_2)=\diy\int h_1(\bx)\log \frac{h_1(\bx)}{h_2(\bx)}{\rm d}\bx.$$
Note that $\Delta$ becomes the KL-divergence
when $h_1$ and $h_2$ are probability density functions.
Furthermore,
\begin{equation}
\diy\sum\limits_{i=1}^m p_i \Delta\big(f_i,f^m\big)=\sum\limits_{i=1}^m \Delta\big(p_i f_i,f^m\big)+H(p). 
\end{equation}
And so,
\begin{equation}\label{eq4.appendix.thm}
\diy\frac{1}{2}\left(H(p)-JS(f_1,f_2,\dots,f_m)\right)=-\diy\frac{1}{2} \sum\limits_{i=1}^m \Delta(p_i f_i,f^m).
\end{equation}
Note that here since $p_if_i\leq f^m$ so $\Delta$ is negative. Next, recall (\ref{JS:lowerbound}) and (\ref{eq4.appendix.thm}) then we can write 
\begin{equation}\begin{array}{l}
\ep^m\geq \diy\frac{1}{4(m-1)}\left(-\sum\limits_{i=1}^m \Delta(p_i,f_i,f^m)\right)^2
\\
\qquad=\diy\frac{1}{4(m-1)}\left(\diy\sum\limits_{i=1}^m \diy\int p_if_i(\bx)\log\diy\frac{f^m(\bx)}{p_if_i(\bx)}\rd\bx\right)^2\\
\\
=\diy\frac{1}{4(m-1)}\left(\diy\sum\limits_{i=1}^m \diy\int p_if_i(\bx)\log\bigg(1+\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{p_if_i(\bx)}\bigg)\rd\bx\right)^2.
\end{array}\end{equation}
In addition, we know that for all $t\geq 0$ we have $\log(1+t)\geq t/(1+t)$. Set $t=\diy\sum\limits_{j\neq i}p_jf_j\Big/p_if_i$, so
\begin{equation}\begin{array}{ccl}
\log\left(1+\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{p_if_i(\bx)}\right)&\geq& \diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{p_if_i(\bx)}\left(1+\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{p_if_i(\bx)}\right)^{-1}\\[10pt]
&=&\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{f^m(\bx)}.
\end{array}\end{equation}
This implies
\begin{equation}
\diy\int p_if_i(\bx)\log\left(1+\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{p_if_i(\bx)}\right)\rd\bx\geq \int {\it p_if_i(\bx)\;\diy\frac{\diy\sum\limits_{j\neq i}p_jf_j(\bx)}{f^m(\bx)}\rd\bx}.
\end{equation}
So the claim is proved.

%---------------------------------------------
\subsection{Theorem \ref{thm2:lowerbound}}
We first need to prove the following Lemma:
\begin{lemma}
\label{lem2}
Let $a_1,a_2,\dots,a_m$ be probability distributions on $m$ classes so $\diy\sum\limits_{i=1}^m a_i=1$. Then 
\begin{equation}\label{lem2.eq.0}
\sqrt{\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m a_ia_j}\leq\diy\sum\limits_{i=1}^{m-1}\sqrt{a_i(1-a_i)}. 
\end{equation}
\end{lemma}
\begin{IEEEproof}
One can easily check that
\begin{equation}\label{thm2.eq1}
\sqrt{\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m a_ia_j}\leq \sqrt{\diy\sum\limits_{i=1}^{m-1}a_i\left(\sum\limits_{j=i+1}^m a_j\right)}\leq\diy\sum\limits_{i=1}^{m-1}\sqrt{a_i\left(\sum\limits_{j=i+1}^m a_j\right)}.
\end{equation}
The RHS in (\ref{thm2.eq1}) is upper bounded by 
\begin{equation}\begin{array}{l}
\diy\sum\limits_{i=1}^{m-1}\sqrt{a_i\left(1-\diy\sum\limits_{j=1}^ia_j\right)}
=\sqrt{a_1(1-a_1)}+\sqrt{a_2(1-a_1-a_2)}\\
\\
\qquad +\dots+\sqrt{a_{m-1}(1-a_1-a_2-\dots-a_{m-1})}\\
\\
\qquad \qquad \leq \sqrt{a_1(1-a_1)}+\sqrt{a_2(1-a_2)}\\
\\
\qquad +\dots+\sqrt{a_{m-1}(1-a_{m-1})}
\leq \diy\sum\limits_{i=1}^{m-1}\sqrt{a_i(1-a_i)}.
\end{array}\end{equation}
This proves the inequality in (\ref{lem2.eq.0}).
\end{IEEEproof}

From (\ref{lem2.eq.0}) in Lemma \ref{lem2} and substitute $p(i|\bx)$ in $a_i$ we can write
\begin{equation}\label{thm2.eq2}
\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m p(i|\bx)p(j|\bx)\leq \left(\diy\sum\limits_{i=1}^{m-1}\sqrt{p(i|\bx)(1-p(i|\bx))}\right)^2.
\end{equation}
Take the expectation from both sides of (\ref{thm2.eq2}) and apply Cauchy inequality, we have 
\begin{equation}\label{thm4.eq.2}
\bbE_{\BX}\left[\diy\sum\limits_{i=1}^{m-1}\sum\limits_{j=i+1}^m p(i|\bx)p(j|\bx)\right]\leq \bbE_{\BX}\left[\left(\diy\sum\limits_{i=1}^{m-1}p(i|\bx)\right)\left(\sum\limits_{i=1}^{m-1}(1-p(i|\bx)\right)\right],
\end{equation}
without lose of generality assume $p(m|\bx)$ is the largest. Then the RHS in (\ref{thm4.eq.2}) is upper bounded by 
\begin{equation}\label{thm4.eq3}
(m-1)\bbE_{\BX}\big[1-p(m|\bx)\big]\leq (m-1)\bbE_{\BX}\left[1-\max\limits_{i}p(i|\bx)\right]=(m-1)\ep^m.
\end{equation}
We know that $$\bbE_{\BX}\left[p(i|\bx)p(j|\bx)\right]=\delta^m_{ij}.$$
Therefore, (\ref{thm4.eq.2}) and (\ref{thm4.eq3}) implies our claim in (\ref{lowerbound.2}). 


==> HP-divergence.tex <==
\section{The Divergence Measure and Generalizations}

In this section we recall the Henze-Penrose (HP) divergence between pairs of densities and define a generalization for multiple densities ($\ge 2$) that will be the basis for learning to bound multi-class BER, called "Generalized HP-integral". 
\subsection{Henze-Penrose Divergence}\label{sec.HP-div}
\def\BX{\mathbf{X}}
For parameters $p\in(0,1)$ and $q=1-p$ consider two density functions $f$ and $g$ with common domain $\mathbb{R}^d$. The Henze-Penrose divergence $D(f,g)$ is given by 
\begin{equation}\label{HP-divergence}
    D(f,g)=\diy\frac{1}{4pq}\left[\int \diy\frac{\big(p f(\bx)-qg(\bx)\big)^2}{pf(\bx)+qg(\bx)}\;{\rm d}\bx-(p-q)^2\right].
\end{equation}
The HP-divergence (\ref{HP-divergence}), first introduced in \cite{BerishaHero2015}, has the following properties: (1) $0\leq D \leq 1$, (2) $D=0$ iff $f(\bx)=g(\bx)$. Note that the HP-divergence belongs to the $f$-divergence family \cite{Csisz1967, AliS1966, Morimoto1963}. 

In the multi-class classification setting, as defined in the introduction, consider a sample of i.i.d. pairs  $(\mathbf{x}_i, y_i)$, $i=1, \ldots, n$, where $y_i \in \{1, \ldots, m\}$ are class labels with prior probabilities $\{p_k\}_{k=1}^m$ and, given $y_i=k$, $\mathbf{x}_i$ has conditional density $f_k$.
%consider $m$ class conditional distributions $f_1,f_2,\dots,f_m$ of an observed random variable $\mathbf{X}$ with class priors $p_1,p_2,\dots,p_{m}\in [0,1]$ such that $$\diy\sum\limits_{k=1}^m p_k=1\;\; \hbox{for}\; i,j=1,2,\dots,m,$$
Define $\widetilde{p}_{ij}=p_i/(p_i+p_j)$. Note that $\widetilde{p}_{ij}\neq \widetilde{p}_{ji}$ and $\widetilde{p}_{ij}+\widetilde{p}_{ji}=1$. Let $\bbS^{(i)}$ be the support set of the conditional distribution $f_i$.  
The Henze-Penrose (HP) divergence measure between distributions $f_{i}$ and $f_{j}$ with union domain $\bbS^{(ij)}=\bbS^{(i)}\cup \bbS^{(j)}$ is defined as follows (see \cite{HP,BerishaHero2015,Berishaetal2016}):
\begin{align}\label{EQ:DP} 
& D(f_{i},f_{j})\nonumber\\
&\quad=\diy\frac{1}{4\widetilde{p}_{ij}\widetilde{p}_{ji}}\Big[\int_{\bbS^{(ij)}} \frac{\big(\widetilde{p}_{ij} f_{i}(\bx)-\widetilde{p}_{ji} f_{j}(\bx)\big)^2}{\widetilde{p}_{ij} f_{i}(\bx)+\widetilde{p}_{ji} f_{j}(\bx)}\;\rd \bx -({\it \widetilde{p}_{ij}-\widetilde{p}_{ji})}^2\Big].
\end{align}
An alternative form for $D(f_{i}, f_{j})$ is given in terms of the HP-integral:
\begin{equation}\label{Def:HP}
{\rm HP}_{ij}:={\rm HP}\big(f_i,f_j\big)=\int_{\bbS^{(ij)}}\diy\frac{f_{i}(\bx)f_{j}(\bx)}{p_i f_{i}(\bx)+p_j f_{j}(\bx)}\rd\bx,\end{equation}
yielding the equivalent form to (\ref{EQ:DP})
$$D(f_{i},f_{j})=1-(p_i+p_j){\rm HP}_{ij}.$$
In \cite{Berishaetal2016} it was shown that $0\leq D(f_{i},f_{j}) \leq 1$, and that the HP-integral is upper bounded by ${\rm HP}\big(f_i,f_j\big)\leq (p_i+p_j)^{-1}$.


\subsection{Generalized HP-Integral}
%Let $\BX^{(i)}=\big\{\BX^{(i)}_1,\dots,\BX^{(i)}_{n_i}\big\}$ 
%Let $\BX^{(i)}$ denote $i$th type of nodes (random vectors) with conditional probability density function $f_i$ and support $\bbS^{(i)}$. For an integer $m\geq 2$, consider $m$-types of nodes $\BX^{(1)},\BX^{(2)}, \dots,\BX^{(m)}$ denoting a random vector $\BX$ with class labels $i=1,2,\dots,m$, $m\geq 2$ respectively.  %with sample sizes $n_1,n_2,\dots,n_m$. 
Define the union of all support sets as $\bbS=\bigcup\limits_{k=1}^m \bbS^{(k)}$ and the difference between the $m$-fold support set and the $2$-fold support set ${\bbS}^{(ij)}$ as $\overline{\bbS}^{(ij)}=\bbS\big/\bbS^{(ij)}$.
%\begin{gather*}
%n=\diy\sum\limits_{s=1}^m n_s, \;\;\bbS=\bigcup\limits_{k=1}^m \bbS^{(k)},\\
%\bbS^{(ij)}=\bbS^{(i)}\cup\;\bbS^{(j)},\;\;  \overline{\bbS}^{(ij)}=\bbS\big/\bbS^{(ij)}.
%\end{gather*}
We denote $f^{(m)}(\bx)$ the marginal distribution of $\BX$,
$$f^{(m)}(\bx):=\diy\sum\limits_{k=1}^m p_k f_{k}(\bx)=\diy\sum\limits_{k=1}^m p_k f(\bx|y=k). $$
Define the generalized HP-integral (GHP-integral) by 
\begin{equation}\label{Def:GHP}
{\rm GHP}^m_{ij}:={\rm GHP}^m\big(f_{i},f_{j}\big)=\diy\int_{\bbS}\diy f_{i}(\bx)f_{j}(\bx)\big/f^{(m)}(\bx)\;\rd\bx.\end{equation}
Note that GHP-integral is not a linear function of a divergence function. Now the question is when a random vector with $m$ class label is considered what is relation between ${\rm HP}_{ij}$ and ${\rm GHP}^m_{ij}$. This explicitly is discussed below.  
%Below we establish a relation between the HP-integral and the GHP-integral. 
\subsection{A Relation Between GHP-Integral and HP-Integral}
%\begin{theorem}\label{thm.1}
Consider conditional probability densities $f_1,f_2,\dots,f_m$ with priors $p_1,p_2,\dots,p_m$ such that $p_1+p_2+\dots+p_m=1$. 
The HP-integral and the GHP-integral are related as follows: 
\begin{itemize}
\item[(a)] If $\left(\bbS^{(i)}\cup\bbS^{(j)}\right)\cap \bigcup\limits_{k\neq i,j}\bbS^{(k)}=\emptyset$, then 
\begin{equation} \label{eq02:thm1} {\rm HP}(f_{i},f_{j})={\rm GHP}^m\big(f_{i},f_{j}\big), \end{equation}
%where $\widetilde{p}_{ij}=p_i\big/(p_i+p_j)$. 
\item[(b)] If $\left(\bbS^{(i)}\cup\bbS^{(j)}\right)\cap \bigcup\limits_{k\neq i,j}\bbS^{(k)}\neq\emptyset$, then there exists a constant C depending only on priors $p_1,p_2,\dots,p_m$ such that 
\begin{equation}\label{eq03:thm1} \diy {\rm HP}(f_{i},f_{j})\leq {\rm GHP}^m\big(f_{i},f_{j}\big)
+\diy C\Big(1-D\Big(\widetilde{p}_{ij}f_i+\widetilde{p}_{ji}f_j,\diy\sum\limits_{k\neq i,j}\widetilde{p}_k^{ij}f_k\Big)\Big), \end{equation}
where $\widetilde{p}_{ij}=p_i/(p_i+p_j)$ and $\widetilde{p}_k^{ij}=p_k\big/\diy\sum\limits_{r\neq i,j}p_r.$
\end{itemize}

%\end{theorem}
The part (a) can be easily derived. The part (b) is shown based on the fact that there exists a constant $C_1$ depending on the $p_i$ and $p_j$ such that for every $f_i$ and $f_j$ 
\begin{equation}\label{equ.thm1}
f_i(\bx)f_j(\bx)\leq C_1\left(p_if_i(\bx)+p_jf_j(\bx)\right)^2, \;\;\hbox{and}
\end{equation}
\begin{equation}
D\Big(\widetilde{p}_{ij}f_i+\widetilde{p}_{ji}f_j,\diy\sum\limits_{k\neq i,j}\widetilde{p}_k^{ij}f_k\Big)=
1-\diy\frac{\diy\int g_{ij}(\bx)\;\rd\bx}{(p_i+p_j)\diy\sum\limits_{r\neq i,j}p_r},
\end{equation}
where $\widetilde{p}_{ij}$ and $\widetilde{p}_{ji}$ are as before, $\widetilde{p}_k^{ij}=p_k\big/\diy\sum\limits_{r\neq i,j}p_r$, and 
\begin{equation}
g_{ij}(\bx):=\diy\left(p_if_i(\bx)+p_jf_j(\bx)\right)\diy\sum\limits_{k\neq i,j}p_kf_k(\bx)\big/f^{(m)}(\bx). 
\end{equation}
The full discussion on relations (\ref{eq02:thm1}) and (\ref{eq03:thm1}) is given in the arXiv version of the paper \cite{arXiv-Paper}. \\
Intuitively we imply that the HP divergence in (\ref{eq03:thm1}) increases when the support set of samples with labels $i$ and $j$ are nearly disjoint from the support sets of the other labels $k\neq i,j$ $k=1,\dots,m$. In this case the HP-integral becomes closer to the GHP-integral. Specially, (\ref{eq03:thm1}) approaches (\ref{eq02:thm1}) as the intersection between support sets $\bbS^{(ij)}$ and $\bigcup\limits_{k\neq i,j}\bbS^{(k)}$ decreases, i.e. the conditional distributions become less overlapping. This in fact validates the relation (7) intuitively. 



